Simplex Decomposition for Portfolio Allocation Constraints in Reinforcement Learning

Portfolio optimization tasks describe sequential decision problems in which the investor's wealth is distributed across a set of assets. Allocation constraints are used to enforce minimal or maximal investments into particular subsets of assets to control for objectives such as limiting the portfolio's exposure to a certain sector due to environmental concerns. Although methods for constrained Reinforcement Learning (CRL) can optimize policies while considering allocation constraints, it can be observed that these general methods yield suboptimal results. In this paper, we propose a novel approach to handle allocation constraints based on a decomposition of the constraint action space into a set of unconstrained allocation problems. In particular, we examine this approach for the case of two constraints. For example, an investor may wish to invest at least a certain percentage of the portfolio into green technologies while limiting the investment in the fossil energy sector. We show that the action space of the task is equivalent to the decomposed action space, and introduce a new reinforcement learning (RL) approach CAOSD, which is built on top of the decomposition. The experimental evaluation on real-world Nasdaq-100 data demonstrates that our approach consistently outperforms state-of-the-art CRL benchmarks for portfolio optimization.

==> figure_5_configuration180181182183192193194195200201202203212213214215220221222223.tex <==
\begin{figure}[H]
\captionsetup[subfigure]{width=0.98\linewidth}
   %%Case 1
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval180181182183.pdf}
    \subcaption{Case 1.1}
    \label{lab:subfigappendixreturnoneone}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting180181182183.pdf}
    \subcaption{Case 1.1}
    \label{lab:subfigappendixconstraintoneone}
   \end{subfigure}

    %%Case 2
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval192193194195.pdf}
    \subcaption{Case 2.1}
    \label{lab:subfigappendixreturntwoone}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting192193194195.pdf}
    \subcaption{Case 2.1}
    \label{placeholderlabelsubfigconstrainttwo}
   \end{subfigure}

    %%Case 3
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval200201202203.pdf}
    \subcaption{Case 3.1}
    \label{lab:subfigappendixreturthreeone}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting200201202203.pdf}
    \subcaption{Case 3.1}
    \label{placeholderlabelsubfigconstraintthree}
   \end{subfigure}


    %%Case 4
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval212213214215.pdf}
    \subcaption{Case 4.1}
    \label{lab:subfigappendixreturnfourone}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting212213214215.pdf}
    \subcaption{Case 4.1}
    \label{placeholderlabelsubfigconstraintfour}
   \end{subfigure}

    %%Case 5
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_legend_inc_interval220221222223.pdf}
    \subcaption{Case 5.1}
    \label{lab:subfigappendixreturnfiveone}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting_legend220221222223.pdf}
    \subcaption{Case 5.1}
    \label{placeholderlabelsubfigconstraintfive}
   \end{subfigure}

\caption{Performance during training; mean total economic payoff and \% of total time steps in violation.}
\label{lab:figureappendixconfigone}
\end{figure}


==> figure_5_configuration224225226227232233234235240241242243248249250251256257258259.tex <==
\begin{figure}[H]
\captionsetup[subfigure]{width=0.98\linewidth}
   %%Case 1
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval224225226227.pdf}
    \subcaption{Case 1.2}
    \label{lab:subfigappendixreturnonetwo}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting224225226227.pdf}
    \subcaption{Case 1.2}
    \label{lab:subfigappendixconstraintonetwo}
   \end{subfigure}

    %%Case 2
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval232233234235.pdf}
    \subcaption{Case 2.2}
    \label{lab:subfigappendixreturntwotwo}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting232233234235.pdf}
    \subcaption{Case 2.2}
    \label{placeholderlabelsubfigconstrainttwo}
   \end{subfigure}

    %%Case 3
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval240241242243.pdf}
    \subcaption{Case 3.2}
    \label{lab:subfigappendixreturthreetwo}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting240241242243.pdf}
    \subcaption{Case 3.2}
    \label{placeholderlabelsubfigconstraintthree}
   \end{subfigure}


    %%Case 4
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval248249250251.pdf}
    \subcaption{Case 4.2}
    \label{lab:subfigappendixreturnfourtwo}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting248249250251.pdf}
    \subcaption{Case 4.2}
    \label{placeholderlabelsubfigconstraintfour}
   \end{subfigure}

    %%Case 5
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_legend_inc_interval256257258259.pdf}
    \subcaption{Case 5.2}
    \label{lab:subfigappendixreturnfivetwo}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting_legend256257258259.pdf}
    \subcaption{Case 5.2}
    \label{placeholderlabelsubfigconstraintfive}
   \end{subfigure}

\caption{Performance during training; mean total economic payoff and \% of total time steps in violation.}
\label{lab:figureappendixconfigtwo}
\end{figure}


==> figure_5_configuration228229230231236237238239244245246247208209210211260261262263.tex <==
\begin{figure}[H]
\captionsetup[subfigure]{width=0.98\linewidth}
   %%Case 1
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval228229230231.pdf}
    \subcaption{Case 1.3}
    \label{lab:subfigappendixreturnonethree}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting228229230231.pdf}
    \subcaption{Case 1.3}
    \label{lab:subfigappendixconstraintonethree}
   \end{subfigure}

    %%Case 2
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval236237238239.pdf}
    \subcaption{Case 2.3}
    \label{lab:subfigappendixreturntwothree}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting236237238239.pdf}
    \subcaption{Case 2.3}
    \label{placeholderlabelsubfigconstrainttwo}
   \end{subfigure}

    %%Case 3
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval244245246247.pdf}
    \subcaption{Case 3.3}
    \label{lab:subfigappendixreturthreethree}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting244245246247.pdf}
    \subcaption{Case 3.3}
    \label{placeholderlabelsubfigconstraintthree}
   \end{subfigure}


    %%Case 4
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_inc_interval208209210211.pdf}
    \subcaption{Case 4.3}
    \label{lab:subfigappendixreturnfourthree}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting208209210211.pdf}
    \subcaption{Case 4.3}
    \label{placeholderlabelsubfigconstraintfour}
   \end{subfigure}

    %%Case 5
   \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/econ_return_plotting_legend_inc_interval260261262263.pdf}
    \subcaption{Case 5.3}
    \label{lab:subfigappendixreturnfivethree}
    \end{subfigure}
    \begin{subfigure}[t]{0.235\textwidth}
     \centering
    \includegraphics[width=\textwidth]{plots/constraint_compliance_plotting_legend260261262263.pdf}
    \subcaption{Case 5.3}
    \label{placeholderlabelsubfigconstraintfive}
   \end{subfigure}

\caption{Performance during training; mean total economic payoff and \% of total time steps in violation.}
\label{lab:figureappendixconfigthree}
\end{figure}


==> figure_5_configuration_only_reward389390391392393394395396397398399400401402403404405406407408455456457458459.tex <==
\begin{figure}
\centering

\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/econ_return_plotting_inc_CI_interval389390391392393.pdf}
  \caption{Case 1.1}
    \label{fig:econreturncaseoneone}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/econ_return_plotting_inc_CI_interval394395396397398.pdf}
  \caption{Case 2.1}
    \label{fig:econreturncasetwoone}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/econ_return_plotting_inc_CI_interval399400401402403.pdf}
  \caption{Case 3.1}
    \label{fig:econreturncasethreeone}
\end{subfigure}

\centering
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/econ_return_plotting_inc_CI_interval404405406407408.pdf}
  \caption{Case 4.1}
   \label{fig:econreturncasefourone}
\end{subfigure}%
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{plots/econ_return_plotting_legend_inc_CI_interval455456457458459.pdf}
  \caption{Case 5.1}
    \label{fig:econreturncasefiveone}
\end{subfigure}

\caption{Five figures arranged in two rows}
\end{figure}






==> tables/constraint_configs/table_experiment_configuration100101102103104105106107108109.tex <==
\begin{table}
	\centering
	\begin{tabular}{C{1.8cm} C{3.6cm} C{1.4cm}}
		\toprule
		& $V_i$ (Affected Assets)& $c_i$ (Constraint Value)\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Experiment 100} & &\\
		Constraint 1& [MSFT, PCAR, NVDA, INTU, EBAY, AMGN, QCOM] & 0.89\\
		Constraint 2& [CASH, NVDA, SBUX, INTU, EBAY] & 0.31\\
		\midrule
		\textbf{Experiment 101} & &\\
		Constraint 1& placeholderconstraintoneone & placeholderconstraintvalueoneone\\
		Constraint 2& placeholderconstrainttwoone & placeholderconstraintvaluetwoone\\
		\midrule
		\textbf{Experiment 102} & &\\
		Constraint 1& placeholderconstraintonetwo & placeholderconstraintvalueonetwo\\
		Constraint 2& placeholderconstrainttwotwo & placeholderconstraintvaluetwotwo\\
		\midrule
		\textbf{Experiment 103} & &\\
		Constraint 1& placeholderconstraintonethree & placeholderconstraintvalueonethree\\
		Constraint 2& placeholderconstrainttwothree & placeholderconstraintvaluetwothree\\
		\midrule
		\textbf{Experiment 104} & &\\
		Constraint 1& placeholderconstraintonefour & placeholderconstraintvalueonefour\\
		Constraint 2& placeholderconstrainttwofour & placeholderconstraintvaluetwofour\\
		\midrule
		\textbf{Experiment 105} & &\\
		Constraint 1& placeholderconstraintonefive & placeholderconstraintvalueonefive\\
		Constraint 2& placeholderconstrainttwofive & placeholderconstraintvaluetwofive\\
		\midrule
		\textbf{Experiment 106} & &\\
		Constraint 1& placeholderconstraintonesix & placeholderconstraintvalueonesix\\
		Constraint 2& placeholderconstrainttwosix & placeholderconstraintvaluetwosix\\
		\midrule
		\textbf{Experiment 107} & &\\
		Constraint 1& placeholderconstraintoneseven & placeholderconstraintvalueoneseven\\
		Constraint 2& placeholderconstrainttwoseven & placeholderconstraintvaluetwoseven\\
		\midrule
		\textbf{Experiment 108} & &\\
		Constraint 1& placeholderconstraintoneeight & placeholderconstraintvalueoneeight\\
		Constraint 2& placeholderconstrainttwoeight & placeholderconstraintvaluetwoeight\\
        \midrule
		\textbf{Experiment 109} & &\\
		Constraint 1& placeholderconstraintonenine & placeholderconstraintvalueonenine\\
		Constraint 2& placeholderconstrainttwonine & placeholderconstraintvaluetwonine\\
		\bottomrule
	\end{tabular}
	\caption{Details of Constraint Configurations for Experiments.}
	\label{tab:constraintconfend}
\end{table}


==> tables/table_5_configuration180181182183192193194195200201202203212213214215220221222223.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{C{1.8cm} C{3.6cm} C{1.4cm}}
		\toprule
		& $V_i$ (Affected Assets)& $c_i$ (Constraint Value)\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 1.1} & &\\
		Constraint 1& [ADBE, PCAR, EBAY, AMGN] & 0.66\\
		Constraint 2& [NVDA, ADP, QCOM] & 0.22\\
		\midrule
		\textbf{Case 2.1} & &\\
		Constraint 1& [ADBE, PCAR, INTU] & 0.87\\
		Constraint 2& [ADBE, PCAR, INTU, ADP] & 0.97\\
		\midrule
		\textbf{Case 3.1} & &\\
		Constraint 1& [MSFT, ADBE, PCAR, NVDA, SBUX, INTU, EBAY, AMGN] & 0.03\\
		Constraint 2& [MSFT, BIDU, ADBE, PCAR, NVDA, INTU, AMGN] & 0.45\\
		\midrule
		\textbf{Case 4.1} & &\\
		Constraint 1& [MSFT, BIDU, ADBE, SBUX] & 0.69\\
		Constraint 2& [CASH, MSFT, ADBE, PCAR, NVDA, SBUX, INTU, ADP, AMZN, EBAY, AMGN, QCOM] & 0.69\\
		\midrule
		\textbf{Case 5.1} & &\\
		Constraint 1& [ADBE, NVDA, SBUX, INTU, AMZN] & 0.73\\
		Constraint 2& [MSFT, SBUX, INTU, AMZN] & 0.56\\
		\bottomrule
	\end{tabular}
	\caption{Details for Configuration Set 1.}
	\label{tab:evaluationinference}
\end{table}


==> tables/table_5_configuration224225226227232233234235240241242243248249250251256257258259.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{C{1.8cm} C{3.6cm} C{1.4cm}}
		\toprule
		& $V_i$ (Affected Assets)& $c_i$ (Constraint Value)\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 1.2} & &\\
		Constraint 1& [MSFT, BIDU, ADBE, SBUX, INTU, ADP, EBAY] & 0.38\\
		Constraint 2& [NVDA, AMZN, QCOM] & 0.21\\
		\midrule
		\textbf{Case 2.2} & &\\
		Constraint 1& [ADBE, AMZN] & 0.27\\
		Constraint 2& [CASH, BIDU, ADBE, INTU, ADP, AMZN, EBAY, AMGN] & 0.87\\
		\midrule
		\textbf{Case 3.2} & &\\
		Constraint 1& [MSFT, PCAR, NVDA, SBUX, INTU, ADP] & 0.15\\
		Constraint 2& [CASH, BIDU, ADBE, NVDA, AMGN, QCOM] & 0.52\\
		\midrule
		\textbf{Case 4.2} & &\\
		Constraint 1& [CASH, BIDU, SBUX, AMGN, QCOM] & 0.68\\
		Constraint 2& [CASH, MSFT, BIDU, ADBE, PCAR, NVDA, INTU, ADP, AMZN, EBAY, AMGN] & 0.64\\
		\midrule
		\textbf{Case 5.2} & &\\
		Constraint 1& [MSFT, BIDU, NVDA, SBUX] & 0.69\\
		Constraint 2& [CASH, MSFT, ADBE, PCAR, NVDA, SBUX, INTU, AMZN, EBAY, AMGN, QCOM] & 0.94\\
		\bottomrule
	\end{tabular}
	\caption{Details for Configuration Set 2.}
	\label{tab:evaluationinference}
\end{table}


==> tables/table_5_configuration228229230231236237238239244245246247252253254255260261262263.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{C{1.8cm} C{3.6cm} C{1.4cm}}
		\toprule
		& $V_i$ (Affected Assets)& $c_i$ (Constraint Value)\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 1.3} & &\\
		Constraint 1& [CASH, MSFT, PCAR, NVDA, INTU, AMZN, AMGN] & 0.73\\
		Constraint 2& [BIDU, ADBE, ADP, EBAY, QCOM] & 0.12\\
		\midrule
		\textbf{Case 2.3} & &\\
		Constraint 1& [ADBE, ADP] & 0.26\\
		Constraint 2& [CASH, BIDU, ADBE, ADP, AMZN, QCOM] & 0.79\\
		\midrule
		\textbf{Case 3.3} & &\\
		Constraint 1& [MSFT, PCAR, INTU, ADP, EBAY, AMGN] & 0.76\\
		Constraint 2& [CASH, MSFT, BIDU, ADBE, NVDA, SBUX, INTU, EBAY] & 0.22\\
		\midrule
		\textbf{Case 4.3} & &\\
		Constraint 1& [CASH, BIDU, NVDA, SBUX, AMZN, EBAY, AMGN, QCOM] & 0.58\\
		Constraint 2& [CASH, MSFT, ADBE, PCAR, NVDA, SBUX, INTU, ADP, EBAY] & 0.8\\
		\midrule
		\textbf{Case 5.3} & &\\
		Constraint 1& [CASH, ADBE, PCAR, NVDA, SBUX, INTU, ADP, AMZN, QCOM] & 0.23\\
		Constraint 2& [CASH, BIDU, ADBE, PCAR, NVDA, SBUX, ADP, AMZN, AMGN, QCOM] & 0.78\\
		\bottomrule
	\end{tabular}
	\caption{Details for Configuration Set 3.}
	\label{tab:evaluationinference}
\end{table}


==> tables/table_hyperparameter_CS1_1_180181182183.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 1.1} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 1.1.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS1_2_224225226227.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 1.2} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 1e-05\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 0.0005\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 1.2.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS1_3_228229230231.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 1.3} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 10\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 1.3.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS2_1_192193194195.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 2.1} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0005\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 1e-05\\
		IPO & \textit{t weight} & 10\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 2.1.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS2_2_232233234235.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 2.2} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 10\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 50\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 2.2.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS2_3_236237238239.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 2.3} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 1e-05\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 5e-05\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 2.3.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS3_1_200201202203.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 3.1} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 5e-05\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 50\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 3.1.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS3_2_240241242243.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 3.2} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 1e-05\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 3.2.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS3_3_244245246247.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 3.3} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 50\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 3.3.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS4_1_212213214215.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 4.1} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0005\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 4.1.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS4_2_248249250251.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 4.2} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 5e-05\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 4.2.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS4_3_208209210211.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 4.3} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0005\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 1e-05\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 4.3.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS5_1_220221222223.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 5.1} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 1e-05\\
		IPO & \textit{t weight} & 10\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 5.1.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS5_2_256257258259.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 5.2} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.001\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 5e-06\\
		IPO & \textit{t weight} & 10\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 20\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 5.2.}
	\label{tab:appendix}
\end{table}

==> tables/table_hyperparameter_CS5_3_260261262263.tex <==
\begin{table}[H]
	\centering
	\begin{tabular}{c C{3.2cm} C{2.4cm} }% C{1.4cm} C{1.4cm}}
		\toprule
		%& \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
		& Parameter & Value\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
		\midrule %Training environment
		\textbf{Case 5.3} & &\\
		RCPO & \text{learning rate} & 5e-06\\
		RCPO & \textit{lambda learning rate} & 0.0005\\
		RCPO & batch size & 4000\\
		RCPO & mini batch size & 128\\
		RCPO & hidden layer size & [512, 256, 128]\\
		\midrule
		IPO & \textit{learning rate} & 1e-05\\
		IPO & \textit{t weight} & 20\\
		IPO & batch size & 4000\\
		IPO & mini batch size & 128\\
		IPO & hidden layer size & [512, 256, 128]\\
		\midrule
        P3O & \textit{learning rate} & 5e-06\\
		P3O & \textit{kappa init} & 50\\
		P3O & batch size & 4000\\
		P3O & mini batch size & 128\\
		P3O & hidden layer size & [512, 256, 128]\\
		\midrule
        CAOSD & \textit{learning rate} & 1e-06\\
		CAOSD & batch size & 4000\\
		CAOSD & mini batch size & 128\\
		CAOSD & hidden layer size & [512, 256, 128]\\
		\bottomrule
	\end{tabular}
	\caption{Hyperparameter settings for Case 5.3.}
	\label{tab:appendix}
\end{table}

==> tables/table_results124125126127128129130131.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c C{1.4cm} C{1.4cm}  C{1.4cm} C{1.4cm}}
 \toprule
  & \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
  & Total econ. payoff (12 months) & Total violations & Total econ. payoff (12 months) & Total violations\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
  \midrule %Training environment
  \textbf{Case 1} & & & &\\
  RCPO& 0.28 & 1 & 0.612 & \textbf{0}\\
  IPO& 0.223 & 12000 & 0.397 & 12\\
  P3O& 0.305 & \textbf{0} & 0.65 & \textbf{0}\\
  ABDO& \textbf{0.425} & \textbf{0} & \textbf{0.881} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 2} & & & &\\
  RCPO& 0.199 & \textbf{0} & 0.311 & \textbf{0}\\
  IPO& 0.2 & 357 & 0.301 & 1\\
  P3O& 0.217 & 8 & 0.3 & \textbf{0}\\
  ABDO& \textbf{0.247} & \textbf{0} & \textbf{0.397} & \textbf{0}\\
\bottomrule
 \end{tabular}
\caption{Evaluation after training is completed. environment~has a total of 12'000 time steps (1000 trajectories), backtesting~has a single trajectory with 12 time steps.}
\label{tab:evaluationinference}
\end{table}

==> tables/table_results180181182183192193194195.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c C{1.4cm} C{1.4cm}  C{1.4cm} C{1.4cm}}
 \toprule
  & \multicolumn{2}{c}{environment} & \multicolumn{2}{c}{backtesting}\\
  & Total econ. payoff (12 months) & Total violations & Total econ. payoff (12 months) & Total violations\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
  \midrule %Training environment
  \textbf{Case 1} & & & &\\
  RCPO& 0.233 & \textbf{0} & 0.334 & \textbf{0}\\
  IPO& 0.209 & 12000 & 0.369 & 12\\
  P3O& 0.238 & 3 & 0.318 & \textbf{0}\\
  ABDO& \textbf{0.331} & \textbf{0} & \textbf{0.536} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 2} & & & &\\
  RCPO& 0.233 & \textbf{0} & 0.419 & \textbf{0}\\
  IPO& 0.214 & 11899 & 0.33 & 12\\
  P3O& 0.269 & \textbf{0} & \textbf{0.486} & \textbf{0}\\
  ABDO& \textbf{0.301} & \textbf{0} & 0.45 & \textbf{0}\\
\bottomrule
 \end{tabular}
\caption{Evaluation after training is completed. environment~has a total of 12'000 time steps (1000 trajectories), backtesting~has a single trajectory with 12 time steps.}
\label{tab:evaluationinference}
\end{table}

==> tables/table_results180181182183192193194195200201202203212213214215220221222223.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c C{1.6cm} C{1.0cm}  C{1.6cm} C{1.0cm}}
 \toprule
  & \multicolumn{2}{c}{\setupAshort} & \multicolumn{2}{c}{\setupBshort}\\
  & Mean total econ. payoff & Total violations & Mean total econ. payoff & Total violations\\[0.5ex] %$\lambda$ \\ [0.5ex] & universally applicable
  \midrule %Training environment
  \textbf{Case 1} & & & &\\
  RCPO& 0.233 & \textbf{0} & 0.334 & \textbf{0}\\
  IPO& 0.209 & 12000 & 0.369 & 12\\
  P3O& 0.238 & 3 & 0.318 & \textbf{0}\\
  CAOSD& \textbf{0.331} & \textbf{0} & \textbf{0.536} & \textbf{0}\\
  Baseline& \textbf{0.179} & \textbf{0} & \textbf{0.104} & \textbf{0} \\
  \midrule %Backtesting
  \textbf{Case 2} & & & &\\
  RCPO& 0.233 & \textbf{0} & 0.419 & \textbf{0}\\
  IPO& 0.214 & 11899 & 0.33 & 12\\
  P3O& 0.269 & \textbf{0} & \textbf{0.486} & \textbf{0}\\
  CAOSD& \textbf{0.301} & \textbf{0} & 0.45 & \textbf{0}\\
  %Baseline& \textbf{0.179} & \textbf{0} & \textbf{0.104} & \textbf{0} \\
  \midrule %Backtesting
  \textbf{Case 3} & & & &\\
  RCPO& 0.37 & \textbf{0} & 0.704 & \textbf{0}\\
  IPO& 0.249 & \textbf{0} & 0.466 & \textbf{0}\\
  P3O& 0.367 & \textbf{0} & 0.718 & \textbf{0}\\
  CAOSD& \textbf{0.383} & \textbf{0} & \textbf{0.746} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 4} & & & &\\
  RCPO& 0.263 & \textbf{0} & 0.412 & \textbf{0}\\
  IPO& 0.242 & \textbf{0} & 0.396 & \textbf{0}\\
  P3O& 0.27 & \textbf{0} & 0.438 & \textbf{0}\\
  CAOSD& \textbf{0.298} & \textbf{0} & \textbf{0.464} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 5} & & & &\\
  RCPO& 0.305 & \textbf{0} & 0.445 & \textbf{0}\\
  IPO& 0.273 & 1 & 0.312 & \textbf{0}\\
  P3O& 0.314 & \textbf{0} & 0.448 & \textbf{0}\\
  CAOSD& \textbf{0.368} & \textbf{0} & \textbf{0.506} & \textbf{0}\\
\bottomrule
 \end{tabular}
\caption{Evaluation after training is completed. \setupAshort~consists of 1000 evaluation trajectories (12000 environment steps), \setupBshort~on the real-world trajectory of 2021.}
\label{tab:evaluationinference}
\end{table}

==> tables/table_results224225226227232233234235240241242243248249250251256257258259.tex <==
\begin{table}[H]
\centering
\begin{tabular}{c C{1.6cm} C{1.0cm}  C{1.6cm} C{1.0cm}}
 \toprule
  & \multicolumn{2}{c}{\setupAshort} & \multicolumn{2}{c}{\setupBshort}\\
  & Mean total econ. payoff & Total violations & Mean total econ. payoff & Total violations\\[0.5ex] %$\lambda$ \\ [0.5ex] & 
  \midrule %Training environment
  \textbf{Case 1.2} & & & &\\
  RCPO& 0.31 & \textbf{0} & \textbf{0.604} & \textbf{0}\\
  IPO& 0.249 & \textbf{0} & 0.363 & \textbf{0}\\
  P3O& 0.293 & 1 & 0.5 & \textbf{0}\\
  CAOSD& \textbf{0.32} & \textbf{0} & 0.556 & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 2.2} & & & &\\
  RCPO& 0.288 & \textbf{0} & 0.248 & \textbf{0}\\
  IPO& 0.281 & \textbf{0} & 0.243 & \textbf{0}\\
  P3O& 0.309 & \textbf{0} & 0.296 & \textbf{0}\\
  CAOSD& \textbf{0.31} & \textbf{0} & \textbf{0.3} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 3.2} & & & &\\
  RCPO& 0.353 & \textbf{0} & 0.695 & \textbf{0}\\
  IPO& 0.213 & \textbf{0} & 0.373 & \textbf{0}\\
  P3O& \textbf{0.379} & \textbf{0} & 0.761 & \textbf{0}\\
  CAOSD& 0.378 & \textbf{0} & \textbf{0.782} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 4.2} & & & &\\
  RCPO& 0.205 & \textbf{0} & 0.227 & \textbf{0}\\
  IPO& 0.159 & \textbf{0} & 0.24 & \textbf{0}\\
  P3O& 0.211 & 60 & 0.273 & \textbf{0}\\
  CAOSD& \textbf{0.247} & \textbf{0} & \textbf{0.295} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 5.2} & & & &\\
  RCPO& 0.35 & \textbf{0} & 0.731 & \textbf{0}\\
  IPO& 0.198 & 12000 & 0.378 & 12\\
  P3O& 0.388 & \textbf{0} & 0.795 & \textbf{0}\\
  CAOSD& \textbf{0.411} & \textbf{0} & \textbf{0.84} & \textbf{0}\\
\bottomrule
 \end{tabular}
\caption{Evaluation after training is completed. \setupAshort~consists of 1000 evaluation trajectories (12000 environment steps), \setupBshort~on the real-world trajectory of 2021.}
\label{tab:evaluationinference}
\end{table}

==> tables/table_results228229230231236237238239244245246247208209210211260261262263.tex <==
\begin{table}[H]
\centering
\begin{tabular}{c C{1.6cm} C{1.0cm}  C{1.6cm} C{1.0cm}}
 \toprule
  & \multicolumn{2}{c}{\setupAshort} & \multicolumn{2}{c}{\setupBshort}\\
  & Mean total econ. payoff & Total violations & Mean total econ. payoff & Total violations\\[0.5ex] %$\lambda$ \\ [0.5ex] & 
  \midrule %Training environment
  \textbf{Case 1.3} & & & &\\
  RCPO& 0.274 & \textbf{0} & 0.482 & \textbf{0}\\
  IPO& 0.218 & \textbf{0} & 0.283 & \textbf{0}\\
  P3O& 0.302 & \textbf{0} & 0.513 & \textbf{0}\\
  CAOSD& \textbf{0.399} & \textbf{0} & \textbf{0.828} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 2.3} & & & &\\
  RCPO& 0.271 & \textbf{0} & 0.319 & \textbf{0}\\
  IPO& 0.228 & \textbf{0} & \textbf{0.37} & \textbf{0}\\
  P3O& \textbf{0.287} & \textbf{0} & 0.366 & \textbf{0}\\
  CAOSD& 0.272 & \textbf{0} & 0.288 & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 3.3} & & & &\\
  RCPO& 0.216 & \textbf{0} & 0.46 & \textbf{0}\\
  IPO& 0.202 & 12000 & 0.339 & 12\\
  P3O& 0.241 & 6 & 0.515 & \textbf{0}\\
  CAOSD& \textbf{0.246} & \textbf{0} & \textbf{0.534} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 4.3} & & & &\\
  RCPO& 0.297 & \textbf{0} & 0.491 & \textbf{0}\\
  IPO& 0.206 & \textbf{0} & 0.317 & \textbf{0}\\
  P3O& 0.284 & \textbf{0} & 0.415 & \textbf{0}\\
  CAOSD& \textbf{0.313} & \textbf{0} & \textbf{0.52} & \textbf{0}\\
  \midrule %Backtesting
  \textbf{Case 5.3} & & & &\\
  RCPO& 0.337 & \textbf{0} & 0.589 & \textbf{0}\\
  IPO& 0.19 & \textbf{0} & 0.264 & \textbf{0}\\
  P3O& 0.341 & \textbf{0} & 0.56 & \textbf{0}\\
  CAOSD& \textbf{0.371} & \textbf{0} & \textbf{0.676} & \textbf{0}\\
\bottomrule
 \end{tabular}
\caption{Evaluation after training is completed. \setupAshort~consists of 1000 evaluation trajectories (12000 environment steps), \setupBshort~on the real-world trajectory of 2021.}
\label{tab:evaluationinference}
\end{table}

==> tables/table_results_average555657585960616263.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.104 & 0.138 & 0.069\\
        IPO& -0.006 & 0.013 & -0.024\\
        P3O& 0.129 & 0.167 & 0.092\\
        CAOSD& 0.144 & 0.173 & 0.115\\
        Baseline& 0.0 & 0.0 & 0.0\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of outperformance of the benchmark approach after training is completed.}
	\label{tab:evaluationaverageinference}
\end{table}

==> tables/table_results_average5556575859606162636465666768697071.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean total economic payoff over baseline & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.11 & 0.133 & 0.087\\
        IPO& 0.001 & 0.016 & -0.013\\
        P3O& 0.131 & 0.156 & 0.107\\
        CAOSD& 0.152 & 0.177 & 0.128\\
        Baseline& 0.0 & 0.0 & 0.0\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of outperformance of the benchmark approach after training is completed.}
	\label{tab:evaluationaverageinference}
\end{table}

==> tables/table_results_average55565758596061626364656667686970717273747576777879808182reward.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.085 & 0.106 & 0.064\\
        IPO& 0.003 & 0.021 & -0.015\\
        P3O& 0.112 & 0.138 & 0.086\\
        CAOSD& 0.125 & 0.147 & 0.103\\
        Baseline& 0.0 & 0.0 & 0.0\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of mean outperformance over Baseline and its 95\% confidence interval in the simulation environment approach for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencereward}
\end{table}

==> tables/table_results_average55565758596061626364656667686970717273747576777879808182reward_bt.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.198 & 0.256 & 0.139\\
        IPO& 0.039 & 0.081 & -0.004\\
        P3O& 0.226 & 0.302 & 0.15\\
        CAOSD& 0.261 & 0.333 & 0.188\\
        Baseline& 0.0 & 0.0 & 0.0\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of mean outperformance over Baseline and its 95\% confidence interval in the backtesting environment approach for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencerewardbt}
\end{table}

==> tables/table_results_average55565758596061626364656667686970717273747576777879808182reward_btdeltabaseline.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.198 & 0.256 & 0.139\\
        IPO& 0.039 & 0.081 & -0.004\\
        P3O& 0.256 & 0.332 & 0.18\\
        CAOSD& 0.261 & 0.333 & 0.188\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of mean outperformance over Baseline and its 95\% confidence interval in the backtesting environment approach for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencerewardbt}
\end{table}

==> tables/table_results_average55565758596061626364656667686970717273747576777879808182rewarddeltabaseline.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.085 & 0.106 & 0.064\\
        IPO& 0.003 & 0.021 & -0.015\\
        P3O& 0.112 & 0.138 & 0.086\\
        CAOSD& 0.125 & 0.147 & 0.103\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of mean outperformance over Baseline and its 95\% confidence interval in the simulation environment approach for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencereward}
\end{table}

==> tables/table_results_average5556575859606162636465666768697071reward.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.11 & 0.133 & 0.087\\
        IPO& 0.001 & 0.016 & -0.013\\
        P3O& 0.131 & 0.156 & 0.107\\
        CAOSD& 0.152 & 0.177 & 0.128\\
        Baseline& 0.0 & 0.0 & 0.0\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of outperformance of the benchmark approach after training is completed.}
	\label{tab:evaluationaverageinference}
\end{table}

==> tables/table_results_average5556575859606162636465666768697071reward_bt.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.246 & 0.318 & 0.174\\
        IPO& 0.012 & 0.052 & -0.027\\
        P3O& 0.286 & 0.373 & 0.199\\
        CAOSD& 0.307 & 0.39 & 0.224\\
        Baseline& 0.0 & 0.0 & 0.0\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of outperformance of the benchmark approach after training is completed.}
	\label{tab:evaluationaverageinference}
\end{table}

==> tables/table_results_average_absolute55565758596061626364656667686970717273747576777879808182reward_btabsoluteperf.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.51 & 0.563 & 0.457\\
        IPO& 0.351 & 0.38 & 0.323\\
        P3O& 0.569 & 0.638 & 0.499\\
        CAOSD& 0.573 & 0.642 & 0.504\\
        Baseline& 0.313 & 0.342 & 0.283\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of mean outperformance over Baseline and its 95\% confidence interval in the backtesting environment approach for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencerewardbtrelativeperf}
\end{table}

==> tables/table_results_average_absolute55565758596061626364656667686970717273747576777879808182rewardabsoluteperf.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{3.2cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& Mean reward over benchmark & +$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$& -$\dfrac{1.96\hat{\sigma}}{\sqrt{n}}$\\[0.5ex]
		\midrule
		RCPO& 0.296 & 0.311 & 0.281\\
        IPO& 0.214 & 0.224 & 0.204\\
        P3O& 0.323 & 0.343 & 0.303\\
        CAOSD& 0.336 & 0.352 & 0.321\\
        Baseline& 0.211 & 0.223 & 0.198\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of mean outperformance over Baseline and its 95\% confidence interval in the simulation environment approach for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencerewardrelativeperf}
\end{table}

==> tables/table_results_average_absolute_merged55565758596061626364656667686970717273747576777879808182absoluteperf.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{1.6cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& $\bar{\theta}^{env}_{app}$ & Upper 95\% CI & Lower 95\% CI\\[0.5ex]
		\midrule
		\textbf{Simulation} & & & \\
		RCPO& 0.296 & 0.311 & 0.281\\
        IPO& 0.214 & 0.224 & 0.204\\
        P3O& 0.313 & 0.333 & 0.294\\
        CAOSD& \textbf{0.336} & 0.352 & 0.321\\
        Baseline& 0.211 & 0.223 & 0.198\\
        \midrule
        \textbf{Backtesting} & & & \\
        RCPO& 0.51 & 0.563 & 0.457\\
        IPO& 0.351 & 0.38 & 0.323\\
        P3O& 0.541 & 0.61 & 0.472\\
        CAOSD& \textbf{0.573} & 0.642 & 0.504\\
        Baseline& 0.313 & 0.342 & 0.283\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of $\bar{\theta}^{env}_{app}$ and its 95\% confidence interval for all approaches in both environments for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferenceabsoluteperf}
\end{table}

==> tables/table_results_average_delta_merged55565758596061626364656667686970717273747576777879808182deltabaseline.tex <==
\begin{table}
	\centering
	\begin{tabular}{c C{1.6cm} C{1.6cm}  C{1.6cm}}
		\toprule
		& $\bar{\delta}^{env}_{app}$ & Upper 95\% CI & Lower 95\% CI\\[0.5ex]
		\midrule
		\textbf{Simulation} & & & \\
		RCPO& 0.085 & 0.106 & 0.064\\
        IPO& 0.003 & 0.021 & -0.015\\
        P3O& 0.102 & 0.128 & 0.076\\
        CAOSD& \textbf{0.125} & 0.147 & 0.103\\
        \midrule
        \textbf{Backtesting} & & & \\
        RCPO& 0.198 & 0.256 & 0.139\\
        IPO& 0.039 & 0.081 & -0.004\\
        P3O& 0.229 & 0.304 & 0.153\\
        CAOSD& \textbf{0.261} & 0.333 & 0.188\\
		\bottomrule
	\end{tabular}
	\caption{Evaluation of $\bar{\delta}^{env}_{app}$ and its 95\% confidence interval for the non-Baseline approaches in both environments for n=28 experiments after training is completed.}
	\label{tab:evaluationaverageinferencedeltabaseline}
\end{table}
